IBEX Observations of Elastic Scattering of Interstellar Helium by Solar Wind Particles

The IBEX-Lo instrument on the Interstellar Boundary Explorer (IBEX) mission observes primary and secondary interstellar helium in its 4 lowest energy steps. Observations of these helium populations have been systematically analyzed and compared to simulations using the analytic full integration of neutrals model (aFINM). A systematic difference is observed between the simulations and observations of secondary helium during solar cycle (SC) 24. We show that elastic scattering of primary helium by solar wind protons, which redistributes atoms from the core of the flux distribution, provides an explanation of the observed divergence from simulations. We verify that elastic scattering forms a halo in the wings of the primary He distribution in the spin-angle direction. Correcting the simulation for the effects of elastic scattering requires an increase of the estimated density of primary helium compared to previous estimates by Ulysses/GAS. Thus, based on our analysis of IBEX observations and $\chi ^2$ minimization of simulation data that include the effects of elastic scattering, any estimation of neutral interstellar helium density at 1 AU by direct detection of the peak flux of neutral helium needs to be adjusted by $~\sim$ 10%

==> sections/Unused/apendix.tex <==
\section{Error Propagation}\label{
sec:apendix}
Firstly we  describe  error propagation for calculating Normalization factors for primary and secondary population. Then for the estimation of error in density which also used in calculating revised normalization factors.
\subsection{Primary and Secondary Population}
While calculating normalization factor for primary population we subtract secondary population but the effect of secondary is negligible as the count rates of primary are in the order of hundreds of secondaries. So the only uncertainty is Poisson uncertainty.
$$
N  = \frac{D}{M} 
$$
$$
\delta N = \frac{\delta D}{M}, \delta D= \frac{\sqrt{c}}{T^2}
$$
c is the count and T is exposure time.

\subsection{Uncertainty for Optimum Parameter by Chi Square Minimization}

We follow the same technique used by \citet{2013ApJ...775...86S} to calculate statistical and propagation error for the optimal parameter estimated by Chi Square Minimization.\\
A chi square can be written as a quadratic function of the varying parameter $A_k$:
$$
\chi ^2 = C_0 +C_2 (A_k-A_k^*)^2
$$
where the best value is $A_k^*$ and $C_0$ is the minimum value of the $\chi ^2$. The total uncertainty of $A_k^*$ is:

$$
\delta A_k^*=\sqrt{\left(\frac{1+C_0/\nu}{C_2}\right)}
$$
where $\nu$ is the degree of freedom.
\subsection{Uncertainty for Revised normalization factor}

Following is the Error Propagation for revised Normalization Factors:
$$
N  = \frac{D}{M} 
$$
$$
N'  = \frac{D}{F \cdot M} = \frac{N}{F} 
$$
$$
\delta N'  = \sqrt{\left( \frac{\partial N'}{\partial F} \delta F \right)^2 + \left( \frac{\partial N'}{\partial N} \delta N \right)^2} 
$$
As $\delta N \sim 0 $ and $\delta N << \delta F$
$$
\delta N'  \sim \frac{N}{F^2} \delta F
$$
 

==> sections/Unused/discussion.tex <==
\section{Discussion}\label{sec:discussion}
While calculating normalization factors we found these factors are lower than 1 at solar maxima for primary population i.e. ecliptic longitude 130-140 and much higher ~ 1.5  for so called secondary orbits in the ecliptic longitude range 80-90. This result indicate that the model estimates higher survival proabability for primaries but 35-45\% lower survival probability for secondary population. This result motivate us to do a bin by bin analysis for the full solar cycle i.e. 2009-2020. In this analysis we perform a trend of some selected bins (13-16) (Spin Angle bin center (72-96 degree from north ecliptic pole NEP) for primary and (12-15) for secondary. The stark comparision between the two is that in solar maxima for the primaries count rate reduced to 45\% in 2015 but for secondaries the minimum occurs at 2012 but start increasing from 2014 onwards. This is true for every relevant bin. This result indicate that the solar activity is not the same for the all interstellar Helium. Here we are only discussing about helium. Hydrogen count rate is affected by the Lyman-alpha intensity over the cycle and their dependancy is out of the scope of this paper.

We compare the data with the simulation and found that the trend is exactly the same for primary and secondary population both but the intensity is different. Where in the normalization factors ranges from 0.95 to 1.05 from 2009 to 2020 for primaries for secondaries it reaches 1.35 averaging over few orbit. For a single orbit it even reaches 3. It clearly suggests that the intensity for secondaries are calculated with some factor missing, this is not the case for primaries.

Charecteristics of secondary population: They are slower than primaries and they come from a higher latitude. As the photoionization rate shows the same pattern it means the calculation of survival probability is not accurate enough. Two properties which are different and important for primaries and secondaries are that they come from a different direction and also they are slow. It gives a hint that the survival probability needs a factor of velocity, which underestimating loss of primaries and overestimating for secondaries.

From bzowski 2008 we already know that the Analytical function used for survival probability in aFNIM is not accurate enough, the rationof  numerically calculated ionization rate to analytical is a  time dependent oscillatory function. But this can not be the only case because it would show the same nature for primary as well. So, the direction and velocity has important significance for photoionization loss. Charge exchange loss 100 times lower than photoionization for helium that’s why we are not interested in that.Another possibilty is in those position we are observing population which are locally produce , and the production rate is higher in solar maxima. But this case is highly unlikely because of the direction and energy of the observed events. 

The photoionization model is accurate enough because it shows the same tendensies over the bins in the given ecliptic range. It means it shows great correlation with data and model.
\begin{figure}[h]
  \centering
 \includegraphics[width=22cm, height=6cm]{plots/photo.eps}
  \caption{Photoionization Rate from 2009 to 2021. The vertical red lines separate different years.}
  \label{fig:your_label}
\end{figure}

\textit{Correlation with Andre's Work}-- Unexpected High intensity of ENA in energy bin 4 and 5 - Andre Galli (2017,2022) pointed out that there is an anomalous strong rise and fall of ENA intensity in the said energy bins in 2015. The cause of this is unknown but it is highly unlikely that this effect arise from the instrument. However, during solar maxima high  background electrons or similar local contamination may be possible. Solar activity reached it’s maxima in 2012, there is a dip in 2013 but again it was almost same intensity in 2014-2015 but the ENA rise is not seen before 2015
We see similar behaviour in esa-2 for 80-90 where the rise is sharp and surprisingly also in the antiram directon for 130-140 but the rise and fall is smooth.


==> sections/Unused/gruntman_scattering.tex <==
 In this study  we use the formulation and assumptions of the aforementioned work and compare its predictions with the observations by IBEX-Lo. We also argue that the increase of the secondary helium flux during solar maximum can be explained by the scattering of primary ISN He by SW protons.

Here, we briefly outline the theoretical formulation employed in this work. The solar wind flux is assumed to be spherically symmetric, characterized by a constant velocity of 450 km/s and a density of 5 $\text{cm}^{-3}$ at 1 AU. Collisions of ISN He with multiply charged oxygen ions  and alpha particles ($<1\%$ and $<4\%$ respectively in SW density) are also possible but are not considered due to their negligible contribution. The scattering of ISN He by SW protons can be treated within a spherically symmetric potential field. This is a reasonable assumption  due to the lower relative velocity between SW protons and ISN He and the internuclear distance between them. This scattering  can be conveniently described in the laboratory frame of reference where the  ISN He is at rest and a proton arrives with a relative velocity $V_r$. In the center of mass frame of reference the scattering angle is $\chi$ and the post-collision velocity gain of He is proportional to the scattering angle. Larger $\chi$  suggest a significant alteration of the ISN He velocity vector. For the elastic differential cross section $\frac{\mathrm{d} \sigma}{\mathrm{d} \Omega}$, the total cross section can be calculated as
\begin{equation}
q_0=2 \pi \int_0^\pi \frac{\mathrm{d} \sigma}{\mathrm{d} \Omega}(\chi) \mathrm{d} \chi,
\end{equation}
which amounts to $6.3 \times 10^{-16} \text{cm}^2 $ at a collision velocity of 450 km/s. This includes scattering for any angle but the large scattering angles resulting from small collision impact parameters lead to the loss of helium atoms through charge exchange ionization.  To differentiate between ionization and scattering, a limiting impact parameter $b_0$ is set to $0.05 \text{\AA}^2$, corresponding to a maximum scattering angle of $\chi \sim 34\degree$. For elastic scattering the impact parameter has to be greater than $b_0$.

Elastic collisions scatter helium atoms towards the wings of the velocity distribution, effectively broadening it. This phenomenon is known as the helium flux halo. The scattered particles are directed in all directions, with two important orientations: along the ecliptic plane and perpendicular to it. IBEX observes these particles at different ecliptic longitudes throughout the year as it orbits in the ecliptic plane. Additionally, for each particular orbit, IBEX scans along swaths perpendicular to the ecliptic plane at different ecliptic latitudes. A crucial assumption in this analysis is that scattering events with angles $\chi <1\degree$ do not produce an observable halo. Consequently, the author considers a minimum scattering angle of $\chi = 1\degree$. For this scattering angle, the author introduces a partial scattering cross-section $q_1$, calculated to be $0.56 \text{\AA}^2$. Using this $q_1$ value, it is  determined that for $\chi \geq 1\degree$, the fraction of atoms experiencing more than one collision is approximately 1/20 of the particles undergoing a single collision. Therefore, it is reasonable to assume that a He atom experiences only a single collision with a SW proton inside the heliosphere.
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{plots/final_paper_plot/gruntman.jpg}
    \caption{Reproduced from \citet{https://doi.org/10.1002/jgra.50199}. The upper panel illustrates the formation of the flux halo in the spin angle swath. The blue line represents the distribution without any collisions, while the green and red dotted lines depict the scenarios with only one collision and none, respectively. The middle and lowest panels display the ratio of the one or none collision approximation with the no collision model, shown in both logarithmic and linear scales. Figure \ref{fig:halo} provides the corresponding observational evidence for  this prediction.}
    \label{fig:gruntman}
\end{figure}

==> sections/Unused/model.tex <==
\section{aFINM}\label{sec:model}
 The study of the distribution function for interstellar neutrals commenced in the 1960s and early 1970s, under the assumption that the interstellar medium is cold \cite{1968Ap&SS...2..474F,1970A&A.....4..280B,1972NASSP.308..609A}. By the late 1970s, researchers such as \citet{1979A&A....77..101F}, \citet{1978AREPS...6..173T}, and \citet{1979ApJ...231..594W} initiated the development of models accounting for the distribution of interstellar hydrogen at finite temperatures. Building upon the hot model, \citet{2012ApJS..198...10L,2015ApJS..220...23L} proposed an analytical model designed to calculate the distribution function of interstellar helium within the heliosphere, specifically adapted to IBEX observations. This model utilizes analytic formulation to calculate survival probability of neutrals based on ionization rate and solar wind flux assuming the ionization rate is constant at a given location and falls off with the inverse square of the heliocentric distance.
 
 \citet{2013ApJ...775...86S} uses this analytical model as a foundation and developed a numerically integrated model where the distribution function is integrated over a detailed response function of IBEX-Lo. The integrations comprise three parts: integration over the spin sector, integration over the collimator, and integration over energy. A more detailed description is available in \citep{,2015ApJS..220...25S}. This model is applied to the goodtime file used for data acquisition. A separate goodtime chunk is used to run the model for every three-hour interval, and eventually, the average count rate is calculated. At the average goodtime position, the real-time spin axis is determined, and based on the input parameters for interstellar helium and hydrogen, the count rates are calculated. 

==> sections/Unused/orbit_by_orbit.tex <==
\section{Orbit by Orbit Analysis}\label{sec:analysis}
\subsection{Different Ecliptic Longitude}
\textit{Longitude 80-90}-- In Ecliptic Longitude 80-90 where the orbit consists mainly secondary population of helium which originates at the boundary of the heliosphere. The solar Activity cycle has a very different effect on these orbits. The solar maxima occurs at 2015 and we also expect that the survival probability of these particles will be lower but we see that in 2015 the count rates in bin 14 reaches to 0.6 /sec. The minima occurs at 2012 around 0.1/sec. Between 2010 and 2013 including there are only one orbit in that longitude, after that there are more than one orbit till 2018. In 2019 and 2020 there are three orbits. The standard deviation is maximum in 2015 as well. If the standard deviation is high it means for a slight change in direction the ENA intensity is different very much. So, in solar maxima 2015 the photoionization is like a stream of UV rays rather than a homogenious irradiation. In contrary for the primary population in 130-140 Ecliptic Longitude, the standard deviation is lower in solar maxima and higher in solar minima.\\

\textit{Longitude 170-180} -- Due to radiation pressure the peak hydrogen occurs much later in the year progression. For primary hydrogen in 170-180 ecliptic longitude the maximum occurs at 2012 and 2013 and the standard deviation is also high. So, it seems that maximum intensity occurs at different time for different longitude. The explanation lies in the speed of these particles and the calculation of survival probability.\\ 

\textit{Longitude 130-140} -- This Longitude zone consists mainly primary helium from the pristine interstellar medium. In 2009 and 2020 in exactly 11 years the average count rates matches at ~ 13/sec. The minima occurs at 2015. In 2011 and 2012 the data is missing. Apparently 2010,2013 and 2014 has almost the same count rate. The standard deviation increases near solar minima again around 2018,2019 and 2020. In 2015 the intensity reduces to 45\% of solar minima in 2009.

\textit{Conclusion}-- The higher values of secondary population in 2015 or primary hydrogen in 2013 is probbaly not a fluke, rather it is a feature of solar UV radiation which affects particle differently. the one question remain is that why the model predicts the same behaviour, it means that from the photoionization rate it is expected. So, everything lies in the calculation of survival probability. The analytical survival probability although flawed it prediction matches with the data very well.

\textit{Justification for 10 degree bin} -- Before orbit 130 the orbits were 7.5 days long and after they were broken into arcs, each arc was 4.5 days long. Each day IBEX moves ~ 1 degree in the ecliptic plane so 10 degree is a good choice. We can also bin the longitude in 5 degree bin but that may lead years of void orbits.

\textit{Calculation of Ecliptic Longitude}-- The Ecliptic Longitude of these orbits are the weighted average over the NonSpunLoBetterTime list which has been described before. If there are n chunks of the bettertime list and $\lambda_i$’s are the ecliptic longitude at the middle of the chunks and $\Delta T_i$’s are the length of the time then $\Lambda=\frac{\sum \lambda_i * \Delta T_i }{\sum \Delta T_i}$
\begin{figure}[h]
  \centering
  \includegraphics[width=20cm, height=6cm]{plots/80_14.png}
  \caption{Your Image Caption}
  \label{fig:your_label}
\end{figure}
\begin{figure}[h]
  \centering
  \includegraphics[width=20cm, height=6cm]{plots/130_14.png}
  \caption{Your Image Caption}
  \label{fig:your_label}
\end{figure}
\begin{figure}[h]
  \centering
  \includegraphics[width=20cm, height=6cm]{plots/170_14.png}
  \caption{Your Image Caption}
  \label{fig:your_label}
\end{figure}


\begin{table}[h]
    \centering
    \begin{minipage}{0.3\linewidth}
        \centering
        \begin{tabular}{|c|c|c|}
            \hline
            \textbf{Year} & \textbf{Code}& \textbf{Longitude} \\
            \hline
            2009 & 0016 & 133.9 \\
            \hline
            2010 & 0063 & 132.1 \\
            2010 & 0064 & 139.4 \\
            \hline
            2013 & 0194b & 130.3 \\
            2013 & 0195a & 134.2 \\
            2013 & 0195b & 137.8 \\
            \hline
            2014 & 0235a & 134.9 \\
            2014 & 0235b & 138.1 \\
            \hline
            2015 & 0275a & 133.4 \\
            2015 & 0275b & 137.6 \\
            \hline
            2016 & 0315a & 132.7 \\
            \hline
            2017 & 0355a & 130.4 \\
            2017 & 0355b & 134.3 \\
            \hline
            2018 & 0395b & 133.6 \\
            2018 & 0396a & 137.7 \\
            \hline
            2019 & 0435b & 130.3 \\
            2019 & 0436a & 134.9 \\
            2019 & 0436b & 138.5 \\
            \hline
            2020 & 0476a & 135.2 \\
            2020 & 0476b & 138.6 \\

            \hline
        \end{tabular}
        \caption{Primary Helium}
        \label{tab:prihel}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.3\linewidth}
        \centering
        \begin{tabular}{|c|c|c|}
            \hline
            \textbf{Year} & \textbf{Orbit} & \textbf{Longitude} \\
            \hline
            2009 & 0057 & 82.0 \\
            2009 & 0058 & 88.9 \\
            \hline
            2010 & 0105 & 82.0 \\
            \hline
            2011 & 0149a & 81.0 \\
            2011 & 0149b & 84.5 \\
            \hline
            2012 & 0189b & 81.8 \\
            2012 & 0190a & 87.5 \\
            \hline
            2013 & 0229b & 83.9 \\
            2013 & 0230a & 88.0 \\
            \hline
            2014 & 0269b & 80.6 \\
            2014 & 0270a & 87.0 \\
            2014 & 0270b & 88.3 \\
            \hline
            2015 & 0310a & 84.6 \\
            2015 & 0310b & 89.6 \\
            \hline
            2016 & 0350a & 83.1 \\
            2016 & 0350b & 85.7 \\
            \hline
            2018 & 0430b & 83.1 \\
            2018 & 0431a & 87.6 \\
            \hline
            2019 & 0470a & 80.3 \\
            2019 & 0470b & 82.0 \\
            2019 & 0471a & 87.0 \\
            \hline
            2020 & 0510b & 81.2 \\
            2020 & 0511a & 85.8 \\
            2020 & 0511b & 89.6 \\
            
            \hline
        \end{tabular}
        \caption{Secondary Helium}
        \label{tab:sechel}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.3\linewidth}
        \centering
        % Include the third table here
        \begin{tabular}{|c|c|c|}
            \hline
            \textbf{Year} & \textbf{Orbit}& \textbf{Longitude} \\
            \hline
            2009 & 0021 & 176.0 \\
            \hline
            2010 & 0069 & 174.4 \\
            \hline
            2011 & 0117 & 177.2 \\
            \hline
            2012 & 0159a & 174.6 \\
            2012 & 0159b & 177.4 \\
            \hline
            2013 & 0199a & 171.3 \\
            2013 & 0199b & 174.4 \\
            \hline
            2014 & 0239b & 172.2 \\
            \hline
            2015 & 0279b & 174.0 \\
            2015 & 0280a & 179.0 \\
            \hline
            2016 & 0319b & 170.0 \\
            \hline
            2017 & 0359b & 170.5 \\
            2017 & 0360a & 177.2 \\
            2017 & 0360b & 179.8 \\
            \hline
            2018 & 0400a & 173.1 \\
            2018 & 0400b & 177.1 \\
            \hline
            2019 & 0440a & 173.0 \\
            2019 & 0440b & 176.3 \\
            \hline
            2020 & 0480b & 175.4 \\  
            \hline
        \end{tabular}
        \caption{Hydrogen}
        \label{tab:hyd}
    \end{minipage}
\end{table}
\textbf{Lo}
{North South Asymmetry}\label{sec:asymmetry}
Show the plot of ratio of North South, which orbit we have chosen and why.


==> sections/Unused/population.tex <==
\section{Results}
\subsection{Temporal variation of scaling factor for different population}\label{sec:norm}
To find the temporal variation of scaling factor at different ecliptic longitudes we use analytical Full Integration Model (aFINM) developed at University of New Hampshire (UNH) which is based on analytical solution of IBEX observation by \citet{2012ApJS..198...10L,2015ApJS..220...23L}  where a full numerical integration technique has been used rather than a  closed form approximation. \\
From here we denote primary and secondary helium by $HE_p$ and $HE_s$ and the respective Normalization factors to be $N_p$ and $N_s$.
Orbits where $He_p$ reaches maximum the ratio of $He_p$ to $HE_s$ is more than 30. In contrary where $He_s$ reaches maximum the ratio of $He_p$ to $He_s$ is typically more than 2. Also the uncertainty of calculating normalization factor for secondary increases 41\% because of the inclusion of $N_p$ It signifies that uncertainty in normalization factor 
 \textit{Normalization Factor} \textemdash The normalization factor or scaling factor for each orbit is  the ratio  of the spin integrated count rates of data and the simulation, \emph{i.e.}  $R=\frac{D_{a}-M_p}{M_{s}}$, $M_p,M_s$ are primary and secondary helium. There are two cases: $R<1$ implies the model underestimate survival probability and $R>1$  the model overestimate survival Probability.\\
 \textit{Survival Probability}  \textemdash Survival Probability is the quantity which measures the detection probability of a interstellar neutral  at 1 AU. 

\begin{table}
    \begin{minipage}{0.5\textwidth}
    %\centering
    \begin{tabular}{ccccccc}\hline
 Year& Orbit& N& Long& SA& Off&Photo\\\hline \hline 
         2012&  0189a&  1.17&  79.23&  -0.11&  5.434& 10.034
\\ \hline 
         2012&  0190a&  0.84&  87.5&  -0.12&  4.774& 10.034
\\ \hline 
         2013&  0191a&  1.25&  97.49&  0.05&  3.836& 9.937
\\ \hline 
         2013&  0191b&  1.78&  101.02&  0.08&  0.964& 9.937
\\ \hline 
 2013& 0192b& 1.37& 110.01& 0.04& 0.316&9.937\\ \hline 
 & & & & & &\\ \hline
    %\end{tabular}
    %\caption{Season 2012-2013}
    %\begin{tabular}{ccccccc} \hline 
         2013&  0229a&  0.7&  79.92&  0.04&  6.097& 10.325\\ \hline 
         2013&  0230a&  0.87&  88.54&  0.7&  3.864& 10.325\\ \hline 
         2013&  0230b&  0.98&  91.37&  0.08&  3.586& 10.325\\ \hline 
         2014&  0231a&  0.85&  98.61&  0.05&  6.38& 10.325\\ \hline 
         2014&  0231b&  1.26&  99.72&  0.02&  0.907& 10.325\\ \hline 
         2014&  0232a&  1.49&  105.95&  -4.75&  4.81& 10.426\\ \hline 
         2014&  0232b&  1.13&  111.15&  -4.97&  5.425& 10.621\\ \hline
         & & & & & &\\
         & & & & & &\\ \hline
    %\end{tabular}
    %\caption{Season 2013-2014}
    %\label{tab:2014}
    %\begin{tabular}{ccccccc} \hline 
         2014&  0269a&  0.9&  76.86&  0.7&  4.547& 11.027
\\ \hline 
         2014&  0270b&  1.45&  88.3&  5.18&  5.184& 11.027
\\ \hline 
         2015&  0271a&  0.78&  95.27&  5.3&  5.544& 11.027
\\ \hline 
         2015&  0271b&  1.18&  98.91&  5.29&  5.441& 11.357
\\ \hline 
         2015&  0272a&  1.29&  106.14&  5.35&  6.217& 11.357\\ \hline
         & & & & & &\\
          & & & & & &\\ \hline
    %\end{tabular}
%\caption{Season 2014-2015}
%\label{tab:2015}
    %\begin{tabular}{ccccccc} \hline 
         2015&  0309a&  0.85&  76.23&  0.06&  5.164& 9.323
\\ \hline 
         2015&  0309b&  0.81&  79.32&  0.01&  1.938& 9.323
\\ \hline 
         2015&  0310a&  0.93&  84.55&  -0.03&  0.747& 9.226
\\ \hline 
         2015&  0310b&  1.97&  87.52&  0.14&  2.61& 9.226
\\ \hline 
         2016&  0311a&  0.98&  95.38&  0&  2.797& 9.226
\\ \hline 
         2016&  0311b&  1.67&  97.64&  0.08&  1.741& 9.226
\\ \hline 
         2016&  0312b&  1.46&  108.03&  0.1&  0.513& 9.226\\ \hline
         %& & & & & &\\ 
        %& & & & & &\\ 
    \end{tabular}
    
    %\caption{Season 2015-2016}
    %\label{tab:2016}
    \end{minipage}
    \hfill
    \begin{minipage}{0.5\textwidth}    
    \begin{tabular}{lccccccc}\hline
  &Year& Orbit& N& Long& SA& Off&Photo\\\hline \hline 
          &2016&  0350a&  0.95&  83.08&  0.1&  2.01& 7.091
\\ \hline 
          &2016&  0350b&  1.21&  85.69&  -0.08&  0.42& 7.091
\\ \hline 
          &2016&  0351a&  1.08&  93.19&  0.08&  2.643& 7.091
\\ \hline 
          &2017&  0351b&  1.29&  96.62&  -0.01&  1.238& 7.091
\\ \hline 
          &2017&  0352a&  1.1&  101.93&  -0.04&  1.771& 6.944
\\ \hline
      && & & & & &\\ \hline
     %\endfirsthead
    %\end{tabular}
    %\caption{Caption}
    %\label{tab:my_label}
        %\begin{tabular}{ccccccc} \hline 
              &2017&  0389b&  1.23&  76.94&  0.01&  2.466& 6.656
\\ \hline 
              &2017&  0391a&  1.02&  92.95&  0.06&  2.988& 6.55
\\ \hline 
              &2018&  0391b&  1.14&  95.06&  0.55&  2.412& 6.55
\\ \hline 
              &2018&  0392a&  1.16&  100.81&  0.02&  1.58& 6.55
\\ \hline 
              &2018&  0392b&  1.26&  105.03&  0.47&  2.78& 6.55
\\ \hline 
              &2018&  0393b&  1.02&  114.85&  0.71&  3.474& 6.55\\ \hline
          && & & & & &\\ \hline
        %\end{tabular}
        %\caption{Caption}
        %\label{tab:my_label}
        %\begin{tabular}{ccccccc} \hline 
              &2018&  0430a&  0.95&  79.74&  0.05&  2.245& 5.897
\\ \hline 
              &2018&  0430b&  1.14&  83.08&  0.09&  1.03& 5.862
\\ \hline 
              &2018&  0431a&  1.21&  87.99&  -0.01&  1.413& 5.862
\\ \hline 
              &2018&  0431b&  1.12&  92.13&  0.51&  2.417& 5.862
\\ \hline 
              &2019&  0432a&  1.05&  97.33&  0.14&  1.414& 5.862
\\ \hline 
              &2019&  0432b&  0.99&  101.82&  0.47&  2.806& 5.862
\\ \hline 
              &2019&  0433a&  1.21&  106.45&  0.1&  1.499& 5.862
\\ \hline 
              &2019&  0433b&  1.16&  111.37&  0.51&  3.256& 5.782\\ \hline
          && & & & & &\\ \hline
        %\end{tabular}
        %\caption{Caption}
        %\begin{tabular}{ccccccc} \hline 
              &2019&  0470a&  0.95&  80.22&  0.01&  3.854& 5.744
\\ \hline 
              &2019&  0470b&  1.13&  81.96&  0.04&  0.821& 5.744
\\ \hline 
              &2019&  0471a&  1.07&  87.02&  0.01&  1.139& 5.744
\\ \hline 
              &2020&  0472a&  1.17&  96.85&  0.08&  1.45& 5.727
\\ \hline 
              &2020&  0472b&  1.29&  101.16&  0.64&  2.08& 5.727
\\ \hline 
              &2020&  0473a&  1.21&  106.49&  0.07&  1.737& 5.727
\\ \hline 
              &2020&  0473b&  1.73&  111.29&  0.41&  2.58& 5.727\\ \hline
        \end{tabular}
     \end{minipage}
     \caption{Orbits used for the different season from 2012-2013 to 2019-2020. Abbreviations: Normalization Factor (N), Ecliptic Longitude of Earth (Long), Spin Axis of IBEX (SA) in degrees, Average Off Pointing of the Orbit in degrees(Off) and Photoionization Rate $* 10^{-7}$ (Photo) }
     \label{table:Orbit Selection}
\end{table}

\textbf{}\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{plots/norms_afterpac1.png}
    \caption{Temporal Evolution of Scaling Factors for Primary and Secondary Population of Interstellar Helium }
    \label{scaling}
\end{figure}
\textit{Variation of Secondary Population}-- Figure \ref{scaling} shows temporal variation of scaling factor for 2013 to 2020. Secondary helium orbits starts at the end of a given year and continues until the end of January, that is why  2013 season includes few orbits from 2012, season 2014 includes few orbits from 2013 and so on. The data before 2013 season is irregular due to unavailability of goodtime. Only 2010 season has significant data but for the continuity of progression season 2010,2011 and 2012 has been excluded from the study.  The PAC voltage was changed in 2012 from 16kV to 7kV which results the efficiency of the instrument by two fold. This change essentially affects the Geometric Factor which has been incorporated in simulation. The scaling factor shows an unusual decrease in 2010 and increase in 2014 in contrast with the primary population of the Interstellar Helium. From 2015 onwards scaling factor steadily increase for the primary but for the secondary it increases sharply till 2017 and becomes almost constant till 2019. However in 2020 it again increases by 6\%.
\subsection{North South Asymmetry}
\begin{figure}[h]
  \centering
  \includegraphics[width=1\linewidth]{plots/nor_so_ratio.eps}
  \caption{Your Image Caption}
  \label{fig:your_label}
\end{figure}
